Multi-band analyses of the bright GRB 230812B and the associated SN2023pel

GRB~230812B is a bright and relatively nearby ($z =0.36$) long gamma-ray burst (GRB) that has generated significant interest in the community and has thus been observed over the entire electromagnetic spectrum. We report over 80 observations in X-ray, ultraviolet, optical, infrared, and sub-millimeter bands from the GRANDMA (Global Rapid Advanced Network for Multi-messenger Addicts) network of observatories and from observational partners. Adding complementary data from the literature, we then derive essential physical parameters associated with the ejecta and external properties (i.e. the geometry and environment) of the GRB and compare with other analyses of this event. We spectroscopically confirm the presence of an associated supernova, SN2023pel, and we derive a photospheric expansion velocity of v $\sim$ 17$\times10^3$ km s$^{-1}$. We analyze the photometric data first using empirical fits of the flux and then with full Bayesian Inference. We again strongly establish the presence of a supernova in the data, with a maximum (pseudo-)bolometric luminosity of $5.75 \times 10^{42}$ erg/s, at $15.76^{+0.81}_{-1.21}$ days (in the observer frame) after the trigger, with a half-max time width of 22.0 days. We compare these values with those of SN1998bw, SN2006aj, and SN2013dx. Our best-fit model favours a very low density environment ($\log_{10}({n_{\rm ISM}/{\rm cm}^{-3}}) = -2.38^{+1.45}_{-1.60}$) and small values for the jet's core angle $\theta_{\rm core} = 1.54^{+1.02}_{-0.81} \ \rm{deg}$ and viewing angle $\theta_{\rm obs} = 0.76^{+1.29}_{-0.76} \ \rm{deg}$. GRB 230812B is thus one of the best observed afterglows with a distinctive supernova bump.

==> SED_results.tex <==
\renewcommand{\arraystretch}{1.4}
\begin{longtable}{cccccccc}
    \label{Table:host220427A}
	\caption[Table]{Summary of SED fitting results. (1) stellar mass in log scale, (2) SFR in log scale, (3) amount of dust attenuation in the V band, (4) metallicity, (5) age weighted by stellar mass, (6) attenuation curve slope for stellar continuum, (7) AGN fraction, (8) mass fraction of the late burst population.} \\ \hline
	%\label{tab:GRBHs_results}
    log$_{10}$(M$_{\star}$) & log$_{10}$(SFR) & A$_V$ & $Z$ & t$_{mass}$ & $\delta$ & $f_{agn}$ & $f_{burst}$ \\
    
	[M$_{\sun}$] & [M$_{\sun}$ yr$^{-1}$] & mag & & Myrs & & & \\ \hline
	\endfirsthead %\hline
$10.62_{-0.32}^{+0.18}$ & $1.89_{-nan}^{+0.31}$ & $1.32\pm0.51$ & $0.004_{-0.004}^{+0.007}$ & $802\pm668$ & $-0.60\pm0.30$ & $0.03_{-0.03}^{+0.06}$ & $0.08_{-0.08}^{+0.08}$ \\ \hline

\end{longtable}

==> cigal_params.tex <==
\begin{table}
	\renewcommand{\arraystretch}{1.2}
	\centering
	\caption{Input parameters for SED fitting with CIGALE}
	\label{Table:paramshost220427A}
	\begin{tabular}{c c c}
	\hline
	Parameter & Symbol & Range \\
	\hline\hline
	{\textbf{Delayed star formation history $+$ recent burst}}\\
	
	Age of the main stellar population & $t_0$ &  200, 500, 1000, 2000, 3000 \,Myrs \\
	E-folding time of the main stellar population model & $\tau$ &  200, 500, 1000, 2000, 3000, 5000, 7000, 10000  Myrs\\
	Mass fraction of the late burst population & $f_{burst}$ &  0.0, 0.1, 0.2\\
	Age of the late burst & $t_b$ &  20.0, 50.0, 100.0, 200.0\\
	E-folding time of the late starburst population & $\tau_{b}$ &  50.0\\
	%Age of the late starburst population & $t_{\rm b}$ &  1, 3, 5, 10, 15, 20, 30, 40, 50, 75, 100 \,Myrs \\
	%e-folding time of the late starburst population model & $\tau_{\rm b}$ &  50, 50000\,Myrs \\
	%Stellar mass fraction due to the burst & $f_{\rm b}$ &  0, 0.01, 0.03, 0.05, 0.075, 0.1, 0.15, 0.20\\
	\hline
	Metallicity $^1$ & $Z$ & 0.0001, 0.008, 0.02\\
    \hline
	{\textbf{Dust attenuation}}\\
	Color excess for nebular emission $^2$ & $\rm E(B-V)_{lines}$ & 0.01, 0.25, 0.5, 0.75, 1.0, 1.25, 1.5, 1.75, 2.0, 2.25, 2.5, 2.75, 3.0 \\
	Ratio of color excess & $\cfrac{E(B-V)_{stars}}{E(B-V)_{lines}}$ & 0.44 \\
	Attenuation curve slope for stellar continuum & $\delta$ & -1, -0.7, -0.4, -0.1, 0.2, 0.5, 0.7\\
	\hline
	{\textbf{AGN$^4$}}\\
	Slope of the power law & $\alpha$ & 2.0\\
	AGN fraction & $f_{agn}$ & 0.0, 0.1, 0.2 \\
	\hline
	Redshift & $z$ & 0.8159 \\
	\hline	
	\hline
	\end{tabular}
	\begin{flushleft}
      \small
      \item $^1$ {$Z$=0.02 being the solar metallicity}
      \item $^2$ {$\rm E(B-V)_{lines}$ is the color excess between the B and V bands applied on the nebular emission lines.}
      \item $^3$ {M$_d$ corresponds to the dust mass heated by the the radiation field intensity U. $\alpha_{IR}$ is fixed to 2 when no IR detection is available.}
      \item $^4$ {Parameters of the dale2014 model \cite{Boquien2019}.}
    \end{flushleft}

\end{table}

==> nmma_posteriors_table_backup.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.1}
    \centering
    \caption{ \texttt{NMMA} - Parameters and prior bounds employed in our Bayesian inferences. We report median posterior values at 95~\% credibility for various physical scenarios and jet structures for the GRB. ``Uniform'' refers to an uniform distribution, and ``LogUniform'' refers to an uniform distribution for the $\log$ of the parameter. $\mathcal{N}(\mu, \sigma^2)$ refers to a Gaussian distribution with mean $\mu$ and variance $\sigma^2$.}
    \label{tab:MCMC_paramsNMMA}
    \begin{turn}{90}
    \resizebox{0.7\paperheight}{!}{
\begin{tabular}{lcccccccccc}
\toprule
& & & \multicolumn{4}{c}{Top-hat} & & & &  \\ \cline{4-7}
Parameter & Prior & Prior range &  & +SN & +Bu2023Ye & +Ka2017 & Gauss & Gauss+SN & Power-law & Power-law+SN \\
\midrule
(log-) Isotropic afterglow energy $E_0$ [erg] & $\rm Uniform$ & $[47, 57]$ & $52.40^{+0.42}_{-0.46}$ & $53.28^{+2.39}_{-1.16}$ & $52.36^{+0.42}_{-0.41}$ & $52.41^{+0.41}_{-0.42}$ & $52.63^{+0.78\phantom{0}}_{-0.58\phantom{0} }$ & $52.60^{+1.90\phantom{0}}_{-0.41\phantom{0} }$ & $52.46^{+0.47\phantom{0}}_{-0.48\phantom{0} }$ & $52.76^{+0.28\phantom{0}}_{-0.26\phantom{0} }$ \\
(log-) Ambient medium's density $n_{\rm ism} $[$\rm{cm}^{-3}$] & $\rm Uniform$ & $[-6, 3]$ & $\myminus4.76^{+1.47}_{-1.17}$ & $\myminus1.68^{+1.57}_{-3.21}$ & $\myminus4.81^{+1.32}_{-1.11}$ & $\myminus4.87^{+1.36}_{-1.06}$ & $\myminus4.66^{+1.65\phantom{0}}_{-1.34\phantom{0} }$ & $\myminus1.41^{+1.25\phantom{0}}_{-2.09\phantom{0} }$ & $\myminus4.78^{+1.46\phantom{0}}_{-1.16\phantom{0} }$ & $\myminus2.16^{+1.21\phantom{0}}_{-1.30\phantom{0} }$ \\
(log-) Energy fraction in electrons $\epsilon_{\mathrm{e}}$ & $\rm Uniform$ & $[-5, 0]$ & $\myminus0.49^{+0.41}_{-0.36}$ & $\myminus0.16^{+0.15}_{-0.56}$ & $\myminus0.53^{+0.38}_{-0.33}$ & $\myminus0.55^{+0.39}_{-0.32}$ & $\myminus0.50^{+0.40\phantom{0}}_{-0.37\phantom{0} }$ & $\myminus0.13^{+0.12\phantom{0}}_{-0.40\phantom{0} }$ & $\myminus0.50^{+0.43\phantom{0}}_{-0.33\phantom{0} }$ & $\myminus0.09^{+0.09\phantom{0}}_{-0.23\phantom{0} }$ \\
(log-) Energy fraction in magnetic field $\epsilon_{\mathrm{B}}$ & $\rm Uniform$ & $[-10, 0]$ & $\myminus0.57^{+0.49}_{-0.90}$ & $\myminus4.40^{+2.07}_{-3.18}$ & $\myminus0.56^{+0.49}_{-0.79}$ & $\myminus0.54^{+0.45}_{-0.83}$ & $\myminus0.66^{+0.57\phantom{0}}_{-1.16\phantom{0} }$ & $\myminus3.56^{+1.60\phantom{0}}_{-2.69\phantom{0} }$ & $\myminus0.55^{+0.48\phantom{0}}_{-0.84\phantom{0} }$ & $\myminus2.44^{+0.83\phantom{0}}_{-0.83\phantom{0} }$ \\
Electron distribution power-law index $p$ & $\rm Uniform$ & $[2.01, 3]$ & $\phantom{0}2.13^{+0.14}_{-0.09}$ & $\phantom{0}2.26^{+0.08}_{-0.20}$ & $\phantom{0}2.14^{+0.12}_{-0.09}$ & $\phantom{0}2.15^{+0.13}_{-0.09}$ & $\phantom{0}2.15^{+0.14\phantom{0}}_{-0.10\phantom{0} }$ & $\phantom{0}2.15^{+0.16\phantom{0}}_{-0.09\phantom{0} }$ & $\phantom{0}2.14^{+0.13\phantom{0}}_{-0.09\phantom{0} }$ & $\phantom{0}2.05^{+0.04\phantom{0}}_{-0.02\phantom{0} }$ \\
Viewing angle $\theta_{\rm obs}$ [degrees] & $\mathcal{N}(0, \theta_{\rm core}^2)$ & -- & $\phantom{0}4.56^{+8.77}_{-4.56}$ & $\phantom{0}2.19^{+2.68}_{-2.00}$ & $\phantom{0}3.40^{+6.23}_{-3.40}$ & $\phantom{0}3.61^{+7.19}_{-3.61}$ & $\phantom{0}8.01^{+11.61}_{-7.99\phantom{0} }$ & $\phantom{0}2.15^{+2.41\phantom{0}}_{-2.08\phantom{0} }$ & $\phantom{0}6.67^{+11.81}_{-6.66\phantom{0} }$ & $\phantom{0}0.75^{+1.27\phantom{0}}_{-0.75\phantom{0} }$ \\
Jet core's opening angle $\theta_{\rm core}$ [degrees] & $\rm Uniform$ & $[0.6, 18]$ & $12.96^{+5.04}_{-6.36}$ & $\phantom{0}3.97^{+4.15}_{-3.38}$ & $13.33^{+4.66}_{-5.73}$ & $13.05^{+4.94}_{-5.83}$ & $10.50^{+7.27\phantom{0}}_{-7.30\phantom{0} }$ & $\phantom{0}3.87^{+2.40\phantom{0}}_{-2.80\phantom{0} }$ & $12.16^{+5.84\phantom{0}}_{-6.78\phantom{0} }$ & $\phantom{0}1.70^{+1.00\phantom{0}}_{-0.71\phantom{0} }$ \\
``Wing'' truncation angle $\theta_{\rm wing}$ [degrees] & $\rm Uniform$ & $[0.6, 45]$ & -- & -- & -- & -- & $28.53^{+16.42}_{-17.77}$ & $25.84^{+19.14}_{-17.70}$ & $28.88^{+16.12}_{-16.47}$ & $20.82^{+18.94}_{-11.93}$ \\
Power-law structure index $b$ & $\rm Uniform$ & $[0.1, 7]$ & -- & -- & -- & -- & -- & -- & $\phantom{0}3.48^{+3.05\phantom{0}}_{-3.37\phantom{0} }$ & $\phantom{0}1.66^{+0.51\phantom{0}}_{-0.42\phantom{0} }$ \\
Angle ratio $\theta_{\rm obs} / \theta_{\rm core}$ & -- & -- & $\phantom{0}0.37^{+0.61}_{-0.35}$ & $\phantom{0}0.55^{+0.25}_{-0.26}$ & $\phantom{0}0.28^{+0.37}_{-0.27}$ & $\phantom{0}0.29^{+0.62}_{-0.29}$ & $\phantom{0}0.99^{+0.99\phantom{0}}_{-0.99\phantom{0} }$ & $\phantom{0}0.65^{+0.42\phantom{0}}_{-0.55\phantom{0} }$ & $\phantom{0}0.61^{+0.98\phantom{0}}_{-0.60\phantom{0} }$ & $\phantom{0}0.44^{+0.76\phantom{0}}_{-0.44\phantom{0} }$ \\
Supernova boost $k_{\rm SN}$ & $\rm Uniform$ & $[0.01, 100]$ & -- & $\phantom{0}1.04^{+0.16}_{-0.17}$ & -- & -- & -- & $\phantom{0}1.05^{+0.15\phantom{0}}_{-0.15\phantom{0} }$ & -- & $\phantom{0}1.04^{+0.09\phantom{0}}_{-0.09\phantom{0} }$ \\
Supernova stretch $s_{\rm SN}$ & $\rm Uniform$ & $[0.1, 5.0]$ & -- & $\phantom{0}0.69^{+0.08}_{-0.07}$ & -- & -- & -- & $\phantom{0}0.69^{+0.07\phantom{0}}_{-0.07\phantom{0} }$ & -- & $\phantom{0}0.68^{+0.05\phantom{0}}_{-0.05\phantom{0} }$ \\
Systematic error $\sigma_{\rm sys}$ & $\rm LogUniform$ & $[0.01, 2.0]$ & $\phantom{0}0.70^{+0.14}_{-0.12}$ & $\phantom{0}0.28^{+0.09}_{-0.08}$ & $\phantom{0}0.71^{+0.14}_{-0.11}$ & $\phantom{0}0.71^{+0.13}_{-0.12}$ & $\phantom{0}0.70^{+0.13\phantom{0}}_{-0.11\phantom{0} }$ & $\phantom{0}0.28^{+0.08\phantom{0}}_{-0.07\phantom{0} }$ & $\phantom{0}0.70^{+0.13\phantom{0}}_{-0.12\phantom{0} }$ & $\phantom{0}0.14^{+0.06\phantom{0}}_{-0.05\phantom{0} }$ \\
\bottomrule
\end{tabular}
}
\end{turn}
\end{table}

==> old_nmma_posteriors_table.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.1}
    \centering
    \caption{ \texttt{NMMA} - Parameters and prior bounds employed in our Bayesian inferences. We report median posterior values at 95~\% credibility for various physical scenarios and jet structures for the GRB. ``Uniform'' refers to an uniform distribution, and ``LogUniform'' refers to an uniform distribution for the $\log$ of the parameter. $\mathcal{N}(\mu, \sigma^2)$ refers to a Gaussian distribution with mean $\mu$ and variance $\sigma^2$.}
    \label{tab:MCMC_paramsNMMA}
    \begin{turn}{90}
    \resizebox{0.7\paperheight}{!}{
\begin{tabular}{lcccccccccc}
\hline
& & & \multicolumn{4}{c}{Top-hat} & & & &  \\ \cline{4-7}
Parameter & Prior & Prior range &  & +SN & +Bu2023Ye & +Ka2017 & Gauss & Gauss+SN & Power-law & Power-law+SN \\
\hline
(log-) Isotropic afterglow energy $E_0$ [erg] & $\rm Uniform$ & $[47, 57]$ & $52.40^{+0.42}_{-0.46}$ & $53.28^{+2.39}_{-1.16}$ & $52.36^{+0.42}_{-0.41}$ & $52.41^{+0.41}_{-0.42}$ & $52.63^{+0.78}_{-0.58 }$ & $52.60^{+1.90}_{-0.41 }$ & $52.46^{+0.47}_{-0.48 }$ & $52.76^{+0.28}_{-0.26 }$ \\
(log-) Ambient medium's density $n_{\rm ism} $[$\rm{cm}^{-3}$] & $\rm Uniform$ & $[-6, 3]$ & $-4.76^{+1.47}_{-1.17}$ & $-1.68^{+1.57}_{-3.21}$ & $-4.81^{+1.32}_{-1.11}$ & $-4.87^{+1.36}_{-1.06}$ & $-4.66^{+1.65}_{-1.34 }$ & $-1.41^{+1.25}_{-2.09 }$ & $-4.78^{+1.46}_{-1.16 }$ & $-2.16^{+1.21}_{-1.30 }$ \\
(log-) Energy fraction in electrons $\epsilon_{\mathrm{e}}$ & $\rm Uniform$ & $[-5, 0]$ & $-0.49^{+0.41}_{-0.36}$ & $-0.16^{+0.15}_{-0.56}$ & $-0.53^{+0.38}_{-0.33}$ & $-0.55^{+0.39}_{-0.32}$ & $-0.50^{+0.40}_{-0.37 }$ & $-0.13^{+0.12}_{-0.40 }$ & $-0.50^{+0.43}_{-0.33 }$ & $-0.09^{+0.09}_{-0.23 }$ \\
(log-) Energy fraction in magnetic field $\epsilon_{\mathrm{B}}$ & $\rm Uniform$ & $[-10, 0]$ & $-0.57^{+0.49}_{-0.90}$ & $-4.40^{+2.07}_{-3.18}$ & $-0.56^{+0.49}_{-0.79}$ & $-0.54^{+0.45}_{-0.83}$ & $-0.66^{+0.57}_{-1.16 }$ & $-3.56^{+1.60}_{-2.69 }$ & $-0.55^{+0.48}_{-0.84 }$ & $-2.44^{+0.83}_{-0.83 }$ \\
Electron distribution power-law index $p$ & $\rm Uniform$ & $[2.01, 3]$ & $2.13^{+0.14}_{-0.09}$ & $2.26^{+0.08}_{-0.20}$ & $2.14^{+0.12}_{-0.09}$ & $2.15^{+0.13}_{-0.09}$ & $2.15^{+0.14}_{-0.10 }$ & $2.15^{+0.16}_{-0.09 }$ & $2.14^{+0.13}_{-0.09 }$ & $2.05^{+0.04}_{-0.02 }$ \\
Viewing angle $\theta_{\rm obs}$ [degrees] & $\mathcal{N}(0, \theta_{\rm core}^2)$ & -- & $4.56^{+8.77}_{-4.56}$ & $2.19^{+2.68}_{-2.00}$ & $3.40^{+6.23}_{-3.40}$ & $3.61^{+7.19}_{-3.61}$ & $8.01^{+11.61}_{-7.99 }$ & $2.15^{+2.41}_{-2.08 }$ & $6.67^{+11.81}_{-6.66 }$ & $0.75^{+1.27}_{-0.75 }$ \\
Jet core's opening angle $\theta_{\rm core}$ [degrees] & $\rm Uniform$ & $[0.6, 18]$ & $12.96^{+5.04}_{-6.36}$ & $3.97^{+4.15}_{-3.38}$ & $13.33^{+4.66}_{-5.73}$ & $13.05^{+4.94}_{-5.83}$ & $10.50^{+7.27}_{-7.30 }$ & $3.87^{+2.40}_{-2.80 }$ & $12.16^{+5.84}_{-6.78 }$ & $1.70^{+1.00}_{-0.71 }$ \\
``Wing'' truncation angle $\theta_{\rm wing}$ [degrees] & $\rm Uniform$ & $[0.6, 45]$ & -- & -- & -- & -- & $28.53^{+16.42}_{-17.77}$ & $25.84^{+19.14}_{-17.70}$ & $28.88^{+16.12}_{-16.47}$ & $20.82^{+18.94}_{-11.93}$ \\
Power-law structure index $b$ & $\rm Uniform$ & $[0.1, 7]$ & -- & -- & -- & -- & -- & -- & $3.48^{+3.05}_{-3.37 }$ & $1.66^{+0.51}_{-0.42 }$ \\
Angle ratio $\theta_{\rm obs} / \theta_{\rm core}$ & -- & -- & $0.37^{+0.61}_{-0.35}$ & $0.55^{+0.25}_{-0.26}$ & $0.28^{+0.37}_{-0.27}$ & $0.29^{+0.62}_{-0.29}$ & $0.99^{+0.99}_{-0.99 }$ & $0.65^{+0.42}_{-0.55 }$ & $0.61^{+0.98}_{-0.60 }$ & $0.44^{+0.76}_{-0.44 }$ \\
Supernova boost $k_{\rm SN}$ & $\rm Uniform$ & $[0.01, 100]$ & -- & $1.04^{+0.16}_{-0.17}$ & -- & -- & -- & $1.05^{+0.15}_{-0.15 }$ & -- & $1.04^{+0.09}_{-0.09 }$ \\
Supernova stretch $s_{\rm SN}$ & $\rm Uniform$ & $[0.1, 5.0]$ & -- & $0.69^{+0.08}_{-0.07}$ & -- & -- & -- & $0.69^{+0.07}_{-0.07 }$ & -- & $0.68^{+0.05}_{-0.05 }$ \\
Systematic error $\sigma_{\rm sys}$ & $\rm LogUniform$ & $[0.01, 2.0]$ & $0.70^{+0.14}_{-0.12}$ & $0.28^{+0.09}_{-0.08}$ & $0.71^{+0.14}_{-0.11}$ & $0.71^{+0.13}_{-0.12}$ & $0.70^{+0.13}_{-0.11 }$ & $0.28^{+0.08}_{-0.07 }$ & $0.70^{+0.13}_{-0.12 }$ & $0.14^{+0.06}_{-0.05 }$ \\
\hline
\end{tabular}}
\end{turn}
\end{table}
